Solving the Real-Time Train Dispatching Problem by Column Generation

Disruptions in the operational flow of rail traffic can lead to conflicts between train movements, such that a scheduled timetable can no longer be realised. This is where dispatching is applied, existing conflicts are resolved and a dispatching timetable is provided. In the process, train paths are varied in their spatio-temporal course. This is called the train dispatching problem (TDP), which consists of selecting conflict-free train paths with minimum delay. Starting from a path-oriented formulation of the TDP, a binary linear decision model is introduced. For each possible train path, a binary decision variable indicates whether the train path is used by the request or not. Such a train path is constructed from a set of predefined path parts (speed-profiles) within a time-space network. Instead of modelling pairwise conflicts, stronger MIP formulation are achieved by a cliques formulated over the complete train path. The combinatorics of speed-profiles and different departure times results in a large number of possible train paths, so that the column generation method is used here. Within the subproblem, the shadow prices of conflict cliques must be taken into account. When constructing a new train path, it must be determined whether this train path belongs to a clique or not. This problem is tackled by a MIP. The methodology is tested on instances from a dispatching area in Germany. Numerical results show that the presented method achieves acceptable computation times with good solution quality while meeting the requirements for real-time dispatching.

==> table/results_complexity_routes.tex <==
\begin{tabular}{c|ccccc} 
	\toprule 
	\diagbox{$n$}{$k$} & 100 & 300 & 500 & 750 & 1000 \\
	\midrule 
	40 & 28.70 / 1148 & 58.65 / 2346 & 76.40 / 3056 & 115.05 / 4602 & 147.90 / 5916 \\
	50 & 25.58 / 1279 & 49.58 / 2479 & 73.58 / 3679 & 103.54 / 5177 & 128.86 / 6443 \\
 	60 & 22.78 / 1367 & 42.78 / 2567 & 62.78 / 3767 & 87.78 / 5267 & 108.88 / 6533 \\
	\bottomrule 
\end{tabular}



==> table/results_complexity_time.tex <==
\begin{tabular}{c|ccccc} 
	\toprule 
	\diagbox{$n$}{$k$} & 100 & 300 & 500 & 750 & 1000 \\
	\midrule 
	40 & 2.6 & 2.06 & 2.32 & 2.63 & 3.86 \\
	50 & 11.8 & 15.65 & 17.54 & 16.56 & 41.08 \\
	60 & 63.66 & 47.38 & 47.6 & 84.16 & 96.62 \\
	\bottomrule 
\end{tabular}


